Fair Correlation Clustering in Forests

The study of algorithmic fairness received growing attention recently. This stems from the awareness that bias in the input data for machine learning systems may result in discriminatory outputs. For clustering tasks, one of the most central notions of fairness is the formalization by Chierichetti, Kumar, Lattanzi, and Vassilvitskii [NeurIPS 2017]. A clustering is said to be fair, if each cluster has the same distribution of manifestations of a sensitive attribute as the whole input set. This is motivated by various applications where the objects to be clustered have sensitive attributes that should not be over- or underrepresented. We discuss the applicability of this fairness notion to Correlation Clustering. The existing literature on the resulting Fair Correlation Clustering problem either presents approximation algorithms with poor approximation guarantees or severely limits the possible distributions of the sensitive attribute (often only two manifestations with a 1:1 ratio are considered). Our goal is to understand if there is hope for better results in between these two extremes. To this end, we consider restricted graph classes which allow us to characterize the distributions of sensitive attributes for which this form of fairness is tractable from a complexity point of view. While existing work on Fair Correlation Clustering gives approximation algorithms, we focus on exact solutions and investigate whether there are efficiently solvable instances. The unfair version of Correlation Clustering is trivial on forests, but adding fairness creates a surprisingly rich picture of complexities. We give an overview of the distributions and types of forests where Fair Correlation Clustering turns from tractable to intractable. The most surprising insight to us is the fact that the cause of the hardness of Fair Correlation Clustering is not the strictness of the fairness condition.

==> proof_matching_forest.tex <==
\begin{lemma}
    Maximum matching in forests can be solved in time in \(\mathcal{O}(n)\).
\end{lemma}
\begin{proof}
    We compute the maximum matchings in the maximal connected components of the forests, that is, the maximal sized trees, independently.
    As there are no edges between these trees, the union of these matchings yields a maximum matching for the forest.
    On each maximal sized tree, we perform a dynamic program as follows. 
    We visit all vertices, but visit each vertex only after we have already visited all its children (for example by employing topological sorting).
    For each vertex \(v\), we compute the maximum matching \(M_v\) in the subtree rooted at \(v\) as well as the maximum matching \(M_v'\) in the subtree rooted at \(v\) assuming \(v\) is not matched.
    We directly get that \(M_v'\) is simply the union of the matchings \(M_u\) for each child \(u\) of \(v\).
    Further, either \(M_v = M_v'\) or in \(M_v\) there is an edge between \(v\) and some child \(u\).
    In the latter case, \(M_v\) is the union of \(\{u,v\}, M_u',\) and the union of all \(M_w\) for all children \(w\neq u\).
    Trying out all possible choices of \(u\) and comparing them among another and to \(M_v'\) yields \(M_v\).
    In the end, the maximum matching in the tree with root \(r\) is \(M_r\).
    
    Each vertex is visited once. 
    If the matchings are not naively merged during the process but only their respective sizes are tracked and the maximum matching is retrieved after the dynamic program by using a back-tracking approach, the time complexity per vertex is linear in the number of its children. 
    Thus, the dynamic program can be computed in time in \(\mathcal{O}(n)\).
\end{proof}
